FastCap: An Efficient and Fair Algorithm for Power Capping in Many-Core Systems

Future servers will incorporate many active lowpower modes for different system components, such as cores and memory. Though these modes provide flexibility for power management via Dynamic Voltage and Frequency Scaling (DVFS), they must be operated in a coordinated manner. Such coordinated control creates a combinatorial space of possible power mode configurations. Given the rapid growth of the number of cores, it is becoming increasingly challenging to quickly select the configuration that maximizes the performance under a given power budget. Prior power capping techniques do not scale well to large numbers of cores, and none of those works has considered memory DVFS. In this paper, we present FastCap, our optimization approach for system-wide power capping, using both CPU and memory DVFS. Based on a queuing model, FastCap formulates power capping as a non-linear optimization problem where we seek to maximize the system performance under a power budget, while promoting fairness across applications. Our FastCap algorithm solves the optimization online and efficiently (low complexity on the number of cores), using a small set of performance counters as input. To evaluate FastCap, we simulate it for a many-core server running different types of workloads. Our results show that FastCap caps power draw accurately, while producing better application performance and fairness than many existing CPU power capping methods (even after they are extended to use of memory DVFS as well).

==> optimization.tex <==
\section{Optimization and algorithms}
We consider the following optimization. 
\begin{align}
\label{eq.obj}
\max &\quad D \\
\label{eq.perfConstraint}
\mbox{s.t.} &\quad \frac{L}{z_i + c_i + R(s_b)} \geq DT_i \quad \forall i \\
\label{eq.powerConstraint}
&\quad \sum_i P_i \left(\frac{\overline{z_i}}{z_i}\right)^{\alpha_i} + P_m \left(\frac{\overline{s_b}}{s_b}\right) + P_{mC} + P_s \leq B \\
\label{eq.minConstraint}
&\quad s_b \geq \overline{s_b}, \quad 0 \leq D \leq 1, \quad z_i \geq \overline{z_i} \quad \forall i 
\end{align}
The objective \eqref{eq.obj} and the constraint \eqref{eq.perfConstraint} try to minimize the performance degradation for the worst core. The parameter $T_i$ is the ``target'' performance that core $i$ is trying to achieve with a degradation of $D$. As will be shown in the next, target $T_i$ is the performance of the baseline system running without any power budget constraint. The idea behind constraint \eqref{eq.perfConstraint} is that each core $i$ should be at least as good as $D$ times its corresponding target $T_i$. It thus maintains the fairness among cores to avoid having some cores receiving too little power budget. We measure the performance in terms of the number of memory accesses each core makes in a given epoch of length $L$. 

The constraint \eqref{eq.powerConstraint} specifies the total power budget for the entire system, taking into account the total core power, memory power and system background power. Constraints \eqref{eq.minConstraint} specify the range of each variable. Since the objective function and each constraint are convex, the optimization problem is convex. 

The optimization problem can be solved quickly in numerical solvers such as CPLEX. However we show some useful theorems which help us to develop an efficient algorithm to find the optimal solution. 

\begin{theorem}
\label{thm.equality}
Suppose the solution $D^*$, $s_b^*$ and $\{z_i^*\}$ are the optimal solution to the optimization problem. Then inequalities \eqref{eq.perfConstraint} and \eqref{eq.powerConstraint} must be equalities.
\end{theorem}

The proof is deferred to the appendix. Theorem~\ref{thm.equality} suggests that the optimal solution must consume the entire power budget and each core must be operating at $D$ times of its corresponding target. With constraints \eqref{eq.perfConstraint} and \eqref{eq.powerConstraint} being equalities, the optimal think time $z_i$ can be solved quickly for a given bus time $s_b$. 

\begin{theorem}
\label{thm.linearZi}
For each given bus transfer time $s_b$, the optimal think time $z_i$ and $D$ conditioned on the given $s_b$ can be determined in linear time $O(N)$.  
\end{theorem}
We defer the proof to the appendix. We note that determining the optimal think time $z_i$ involves a binary search on the range of $D$, i.e., $[0, 1]$. Often one can discretize the interval $[0, 1]$ such that $D$ can take a finite amount of values. 

Theorem~\ref{thm.linearZi} suggests that one can exhaustively search through all bus transfer times to find the optimal solution. However we note that since the optimization problem is convex, we only need to find a local optimal. Also since for each bus transfer time $s_b$ we can find the conditional optimal solution, we can simply perform a binary search on all $M$ possible values $s_b$ can take to find the local optimal. This results in an $O(N \log M)$ algorithm with its pseudo-code shown in Algorithm~\ref{alg.alg1}. 

\begin{algorithm}
\caption{\powerscale~$O(N \log M)$ Algorithm}
\label{alg.alg1}
\begin{algorithmic}[1]
\STATE Let $\ell = 0$, $r = M-1$ and $m = (\ell + r) / 2$.
\WHILE {$\ell \neq r$}
\STATE $m = (\ell+r) / 2$.
\STATE Solve the optimal $D$ for the $m^{th}$ $s_b$ value.
\STATE Solve the optimal $D$ for the $(m \pm 1)^{th}$ $s_b$ values. Let the optimal $D$ be denoted as $D^+$ and $D^-$ respectively. 
\IF {$D < D^+$}
\STATE $\ell = m$
\ELSIF {$D^- > D$}
\STATE $r = m$
\ELSE
\STATE {\bf break} 
\ENDIF
\ENDWHILE 
\STATE Return the optimal solution with the maximum $D$.
\end{algorithmic}
\end{algorithm}

